Utilizing Explainable AI for Quantization and Pruning of Deep Neural Networks

For many applications, utilizing DNNs (Deep Neural Networks) requires their implementation on a target architecture in an optimized manner concerning energy consumption, memory requirement, throughput, etc. DNN compression is used to reduce the memory footprint and complexity of a DNN before its deployment on hardware. Recent efforts to understand and explain AI (Artificial Intelligence) methods have led to a new research area, termed as explainable AI. Explainable AI methods allow us to understand better the inner working of DNNs, such as the importance of different neurons and features. The concepts from explainable AI provide an opportunity to improve DNN compression methods such as quantization and pruning in several ways that have not been sufficiently explored so far. In this paper, we utilize explainable AI methods: mainly DeepLIFT method. We use these methods for (1) pruning of DNNs; this includes structured and unstructured pruning of \ac{CNN} filters pruning as well as pruning weights of fully connected layers, (2) non-uniform quantization of DNN weights using clustering algorithm; this is also referred to as Weight Sharing, and (3) integer-based mixed-precision quantization; this is where each layer of a DNN may use a different number of integer bits. We use typical image classification datasets with common deep learning image classification models for evaluation. In all these three cases, we demonstrate significant improvements as well as new insights and opportunities from the use of explainable AI in DNN compression.

==> Makefile <==
################################################################################
# Settings
################################################################################

COMPILER := pdflatex
BIBTEXER := biber

DOCUMENT   = paper
REFERENCES = paper.bib
#FONTS      = Myriad Minion

PDFDEP := $(wildcard *.tex) \
          $(wildcard head/*.tex) \
          $(wildcard body/*.tex) \
          $(wildcard code/*) \
          $(wildcard figures/*.tex)


################################################################################
# Variables
################################################################################

TEXINPUTS := ./theme/:$(TEXINPUTS)
COMPILER  := TEXINPUTS=$(TEXINPUTS) $(COMPILER)

ifdef FONTS
  TEXMFLOCAL := $(shell kpsewhich -var-value TEXMFLOCAL)
endif

ifndef VERBOSE
  PIPE     := 1>/dev/null 2>/dev/null
  INDENT   := 2>&1 | sed 's/^/    /'
  COMPILER := $(COMPILER) -interaction=nonstopmode
endif

ifdef REFERENCES
  BIBDEP := $$@.bbl
endif


################################################################################
# Functions
################################################################################

check_error = \
  if [ ! $(1) -eq 0 ]; then \
    cat $(2).log | \
      perl -0777 -ne 'print m/\n! .*?\nl\.\d.*?\n.*?(?=\n)/gs' $(INDENT); \
    exit 1; \
  fi

compile = $(COMPILER) -shell-escape $(1).tex $(PIPE) || \
            $(call check_error, $$?, $(1))


################################################################################
# Targets
################################################################################

.PHONY: all $(DOCUMENT) clean distclean
.PRECIOUS: %.pdf %.bcf %.bbl
.SECONDEXPANSION:

all: $(DOCUMENT)

status:
	@echo "Building $(DOCUMENT).pdf"

# .tex -> .pdf and .bcf
%.pdf %.bcf: %.tex $(PDFDEP) | status
	@# Initial compile
	@echo "  Compiling $*.tex"
	@$(call compile, $*)

# .bcf -> .bbl
%.bbl: %.bcf $(REFERENCES) | status
	@# Bibliography
	@echo "  Running $(BIBTEXER)"
	-@$(BIBTEXER) $* $(PIPE)
	@# Update references
	@echo "  Updating references"
	@$(call compile, $*)
	@# Reset time stamp of .bbl to newer than .bcf
	@touch $@

$(DOCUMENT): $$@.pdf $(BIBDEP)
	@# Fill in missing references
	@if test -e $@.log \
	      && ( grep -q "There were undefined references." $@.log \
	        || grep -q "Rerun to get outlines right" $@.log ); then  \
	  echo "  Filling in missing references"; \
	  $(call compile, $@); \
	fi
	@# Fix cross-references
	@while test -e $@.log \
	      && grep -q "Rerun to get cross-references right." $@.log; do \
	  echo "  Fixing cross-references"; \
	  $(call compile, $@); \
	done

ifdef FONTS
fontinstall:
	@for f in $(FONTS); do \
	  echo "Installing font $$f to $(TEXMFLOCAL)"; \
	  sudo cp -r fonts/$$f/* $(TEXMFLOCAL) $(PIPE); \
	  if [ ! $$? -eq 0 ]; then exit 1; fi; \
	done
	@sudo $$(which mktexlsr)
	@for f in $(FONTS); do \
	  echo "Enabling font $$f"; \
	  updmap -user --disable $$f.map $(PIPE); \
	  updmap -user --enable Map=$$f.map $(PIPE); \
	  if [ ! $$? -eq 0 ]; then exit 1; fi; \
  done
endif

# Create a single source version, which is useful for some journals
single: $(PDFDEP) $(REFERENCES)
	@echo "Creating single source version"
	@# Call Latexpand to create a single source file
	@echo "  Running Latexpand"
	@latexpand --keep-comments $(DOCUMENT).tex -o $@.tex $(PIPE)
	@# Search library includes and replace by a single unified include
	@echo "  Patching TikZ and PGFPlots library includes"
	@for LIB in tikz pgfplots; do \
	  grep use$${LIB}library $@.tex | \
	    sed 's/\\use'$${LIB}'library{\(.*\)}/\1/g' | tr -d ' ' | \
	    sed 's/,/\n/g' | sort | uniq | xargs | tr ' ' ',' > libs.$${LIB}; \
	  sed -i '/use'$${LIB}'library.*/d' $@.tex; \
	  if [ -s libs.$${LIB} ]; then \
	    sed -i 's/\(\\usepackage{'$${LIB}'}\)/\1\n\\use'$${LIB}'library{'$$(cat libs.$${LIB})'}/g' $@.tex; \
	  fi; \
	  rm -f libs.$${LIB}; \
	done
	@# Create output folder and stage all files into it
	@echo "  Staging files to '$@'"
	@mkdir -p $@
	@rsync -a * $@/ --exclude $@ $(PIPE)
	@mv $@.tex $@/$(DOCUMENT).tex
	@# Delete dependent TeX files and resulting empty folders
	@echo "  Cleanup"
	@cd $@; rm $@.tex $$(echo "$(PDFDEP)" | \
	  sed 's/\ /\n/g' | grep "tex$$" | grep -v "$(DOCUMENT).tex" | xargs)
	@find $@/ -type d -empty ! -path "$@/figures" -delete

clean:
	rm -rf *.aux *.auxlock *.ind *.idx *.toc *.out *.log *.lot *.ilg *.dvi *.bbl \
	  *.blg *.sub *.suc *.syc *.sym *.syg *.syi *.synctex *.slg *.lol *.lof \
	  *.ist *.gls *.glo *.gli *.glg *.alg *.acr *.acn *.ps *.defn *.nlo *.satz \
	  *.nav *.snm *.xml *.synctex.gz *.synctex *.vrb *.bcf *.makefile *.figlist \
	  $$(ls figures/$(DOCUMENT)-figure[0-9]*.* 2>/dev/null | grep -v pdf) single

distclean: clean
	rm -f $(DOCUMENT).pdf figures/$(DOCUMENT)-figure[0-9]*.* paper-figures/$(DOCUMENT)-figure[0-9]*.*



==> figures/LocalPruning.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}[scale=0.50,transform shape]
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(1.05,0.40)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={prune\_amount},
xmin=-0.024, xmax=0.944,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={accuracy},
ymin=0.0414596619897959, ymax=1.02935507015306,
ytick style={color=black}
]
\addlegendimage{line legend,color0}
\addlegendentry{\( \ell_1 \)-norm}
\addlegendimage{line legend,color1}
\addlegendentry{DeepLIFT}
\addlegendimage{line legend,color2}
\addlegendentry{Conductance}

\addlegendimage{black,mark=diamond}
\addlegendentry{layer 21}
\addlegendimage{black,mark=square}
\addlegendentry{layer 16-21}
\addplot [semithick, color0, mark=square*, mark size=3, mark options={solid,draw=white}, forget plot]
table {%
0.02 0.857194674744898
0.04 0.310092474489796
0.08 0.264787946428571
0.16 0.126518654336735
0.32 0.142239317602041
0.5 0.1109375
0.64 0.0863639987244898
0.8 0.095149075255102
0.9 0.100358737244898
};
\addplot [semithick, color0, dash pattern=on 4pt off 1.5pt, mark=diamond*, mark size=3, mark options={solid,draw=white}, forget plot]
table {%
0.02 0.983573820153061
0.04 0.984036192602041
0.08 0.982876275510204
0.16 0.983346619897959
0.32 0.976965082908163
0.5 0.954053730867347
0.64 0.931385522959184
0.8 0.666788903061225
0.9 0.418347417091837
};
\addplot [semithick, color1, mark=square*, mark size=3, mark options={solid,draw=white}, forget plot]
table {%
0.02 0.976122921994885
0.04 0.925331681585678
0.08 0.83224104859335
0.16 0.707061221227621
0.32 0.49750239769821
0.5 0.161185262148338
0.64 0.188359175191816
0.8 0.101402653452685
0.9 0.100023976982097
};
\addplot [semithick, color1, dash pattern=on 4pt off 1.5pt, mark=diamond*, mark size=3, mark options={solid,draw=white}, forget plot]
table {%
0.02 0.983395939897698
0.04 0.981917359335038
0.08 0.984115249360614
0.16 0.982916400255754
0.32 0.980119085677749
0.5 0.978420716112532
0.64 0.971447410485934
0.8 0.935841592071611
0.9 0.492287404092072
};
\addplot [semithick, color2, mark=square*, mark size=3, mark options={solid,draw=white}, forget plot]
table {%
0.02 0.948385682397959
0.04 0.9416015625
0.08 0.824366230867347
0.16 0.63941725127551
0.32 0.467362882653061
0.5 0.230086096938775
0.64 0.10230787627551
0.8 0.129432397959184
0.9 0.100219228316327
};
\addplot [semithick, color2, dash pattern=on 4pt off 1.5pt, mark=diamond*, mark size=3, mark options={solid,draw=white}, forget plot]
table {%
0.02 0.983107461734694
0.04 0.983537946428571
0.08 0.984450733418367
0.16 0.982991868622449
0.32 0.979795121173469
0.5 0.975402582908163
0.64 0.971480389030612
0.8 0.963420758928571
0.9 0.494997608418367
};
\end{axis}

\end{tikzpicture}


==> figures/NipsFlopsMacs.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{groupplot}[group style={group size=2 by 1}]
\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
title={alexnet},
x grid style={white!69.0196078431373!black},
xmin=-0.595, xmax=8.095,
xtick style={color=black},
xtick={0.5,1.5,2.5,3.5,4.5,5.5,6.5,7.5},
xticklabel style = {rotate=40.0},
xticklabels={conv1,conv2,conv3,conv4,conv5,fc1,fc2,fc3},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=1.05,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:0.3,0) rectangle (axis cs:0.7,0.227405247813411);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{MACs}

\draw[draw=none,fill=color0] (axis cs:1.3,0) rectangle (axis cs:1.7,1);
\draw[draw=none,fill=color0] (axis cs:2.3,0) rectangle (axis cs:2.7,0.33383295369042);
\draw[draw=none,fill=color0] (axis cs:3.3,0) rectangle (axis cs:3.7,0.500677015578214);
\draw[draw=none,fill=color0] (axis cs:4.3,0) rectangle (axis cs:4.7,0.333784677052143);
\draw[draw=none,fill=color0] (axis cs:5.3,0) rectangle (axis cs:5.7,0.0842447334186887);
\draw[draw=none,fill=color0] (axis cs:6.3,0) rectangle (axis cs:6.7,0.0374421037416394);
\draw[draw=none,fill=color0] (axis cs:7.3,0) rectangle (axis cs:7.7,0.00914113860879869);
\draw[draw=none,fill=color1] (axis cs:-0.2,0) rectangle (axis cs:0.2,0.00092315673828125);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
\addlegendentry{NPs}

\draw[draw=none,fill=color1] (axis cs:0.8,0) rectangle (axis cs:1.2,0.0162760416666667);
\draw[draw=none,fill=color1] (axis cs:1.8,0) rectangle (axis cs:2.2,0.0234375);
\draw[draw=none,fill=color1] (axis cs:2.8,0) rectangle (axis cs:3.2,0.03515625);
\draw[draw=none,fill=color1] (axis cs:3.8,0) rectangle (axis cs:4.2,0.0234375);
\draw[draw=none,fill=color1] (axis cs:4.8,0) rectangle (axis cs:5.2,1);
\draw[draw=none,fill=color1] (axis cs:5.8,0) rectangle (axis cs:6.2,0.444444444444444);
\draw[draw=none,fill=color1] (axis cs:6.8,0) rectangle (axis cs:7.2,0.108506944444444);

\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
title={vgg16},
x grid style={white!69.0196078431373!black},
xmin=-0.995, xmax=16.495,
xtick style={color=black},
xtick={0.5,1.5,2.5,3.5,4.5,5.5,6.5,7.5,8.5,9.5,10.5,11.5,12.5,13.5,14.5,15.5},
xticklabel style = {rotate=40.0},
xticklabels={conv1,conv2,conv3,conv4,conv5,conv6,conv7,conv8,conv9,conv10,conv11,conv12,conv13,fc1,fc2,fc3},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=1.05,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:0.3,0) rectangle (axis cs:0.7,0.048526863084922);
\draw[draw=none,fill=color0] (axis cs:1.3,0) rectangle (axis cs:1.7,1);
\draw[draw=none,fill=color0] (axis cs:2.3,0) rectangle (axis cs:2.7,0.5);
\draw[draw=none,fill=color0] (axis cs:3.3,0) rectangle (axis cs:3.7,0.999133448873484);
\draw[draw=none,fill=color0] (axis cs:4.3,0) rectangle (axis cs:4.7,0.499566724436742);
\draw[draw=none,fill=color0] (axis cs:5.3,0) rectangle (axis cs:5.7,0.998700173310225);
\draw[draw=none,fill=color0] (axis cs:6.3,0) rectangle (axis cs:6.7,0.998700173310225);
\draw[draw=none,fill=color0] (axis cs:7.3,0) rectangle (axis cs:7.7,0.499350086655113);
\draw[draw=none,fill=color0] (axis cs:8.3,0) rectangle (axis cs:8.7,0.998483535528596);
\draw[draw=none,fill=color0] (axis cs:9.3,0) rectangle (axis cs:9.7,0.998483535528596);
\draw[draw=none,fill=color0] (axis cs:10.3,0) rectangle (axis cs:10.7,0.249620883882149);
\draw[draw=none,fill=color0] (axis cs:11.3,0) rectangle (axis cs:11.7,0.249620883882149);
\draw[draw=none,fill=color0] (axis cs:12.3,0) rectangle (axis cs:12.7,0.249620883882149);
\draw[draw=none,fill=color0] (axis cs:13.3,0) rectangle (axis cs:13.7,0.0554592720970537);
\draw[draw=none,fill=color0] (axis cs:14.3,0) rectangle (axis cs:14.7,0.00905457503625367);
\draw[draw=none,fill=color0] (axis cs:15.3,0) rectangle (axis cs:15.7,0.00221058960846037);
\draw[draw=none,fill=color1] (axis cs:-0.2,0) rectangle (axis cs:0.2,1.68158083545918e-05);
\draw[draw=none,fill=color1] (axis cs:0.8,0) rectangle (axis cs:1.2,0.000358737244897959);
\draw[draw=none,fill=color1] (axis cs:1.8,0) rectangle (axis cs:2.2,0.000717474489795918);
\draw[draw=none,fill=color1] (axis cs:2.8,0) rectangle (axis cs:3.2,0.00143494897959184);
\draw[draw=none,fill=color1] (axis cs:3.8,0) rectangle (axis cs:4.2,0.00286989795918367);
\draw[draw=none,fill=color1] (axis cs:4.8,0) rectangle (axis cs:5.2,0.00573979591836735);
\draw[draw=none,fill=color1] (axis cs:5.8,0) rectangle (axis cs:6.2,0.00573979591836735);
\draw[draw=none,fill=color1] (axis cs:6.8,0) rectangle (axis cs:7.2,0.0114795918367347);
\draw[draw=none,fill=color1] (axis cs:7.8,0) rectangle (axis cs:8.2,0.0229591836734694);
\draw[draw=none,fill=color1] (axis cs:8.8,0) rectangle (axis cs:9.2,0.0229591836734694);
\draw[draw=none,fill=color1] (axis cs:9.8,0) rectangle (axis cs:10.2,0.0229591836734694);
\draw[draw=none,fill=color1] (axis cs:10.8,0) rectangle (axis cs:11.2,0.0229591836734694);
\draw[draw=none,fill=color1] (axis cs:11.8,0) rectangle (axis cs:12.2,0.0229591836734694);
\draw[draw=none,fill=color1] (axis cs:12.8,0) rectangle (axis cs:13.2,1);
\draw[draw=none,fill=color1] (axis cs:13.8,0) rectangle (axis cs:14.2,0.163265306122449);
\draw[draw=none,fill=color1] (axis cs:14.8,0) rectangle (axis cs:15.2,0.039859693877551);
\end{groupplot}

\end{tikzpicture}


==> figures/WeightSharing.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}[scale=0.50]
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{groupplot}[group style={group size=2 by 1}]
\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={n\_bits},
xmajorgrids,
xmin=1, xmax=5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={accuracy},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black}
]
\addplot [semithick, color0, mark=square*, mark size=3, mark options={solid,draw=white}, forget plot]
table {%
1 0.107727635782748
2 0.292432108626198
3 0.745107827476038
4 0.900359424920128
5 0.917531948881789
};
\addplot [semithick, color1, dash pattern=on 4pt off 1.5pt, mark=diamond*, mark size=3, mark options={solid,draw=white}, forget plot]
table {%
1 0.120607028753994
2 0.212460063897764
3 0.805411341853035
4 0.902056709265176
5 0.920327476038339
};
\addplot [semithick, color2, dash pattern=on 1pt off 1pt, forget plot]
table {%
1 0.1
2 0.3
3 0.76
4 0.9
5 0.92
};

\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={n\_bits},
xmajorgrids,
xmin=1, xmax=5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black}
]
\path [draw=color2, fill=color2, opacity=0.2]
(axis cs:1,0.1)
--(axis cs:1,0.1)
--(axis cs:1,0.1)
--(axis cs:1,0.1)
--cycle;

\addplot [semithick, color0, mark=square*, mark size=3, mark options={solid,draw=white}, forget plot]
table {%
1 0.0998402555910543
2 0.116413738019169
3 0.283845846645367
4 0.690894568690096
5 0.899960063897764
};
\addplot [semithick, color1, dash pattern=on 4pt off 1.5pt, mark=diamond*, mark size=3, mark options={solid,draw=white}, forget plot]
table {%
1 0.09375
2 0.100239616613419
3 0.334464856230032
4 0.861521565495208
5 0.914836261980831
};
\addplot [semithick, color2, dash pattern=on 1pt off 1pt, forget plot]
table {%
1 0.1
2 0.1
3 0.2
4 0.8
5 0.9
};
\end{groupplot}

\end{tikzpicture}


==> figures/resnet_cifar.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\begin{groupplot}[group style={group size=2 by 2}]
\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.97,0.03)}, anchor=south east, draw=white!80!black},
tick align=outside,
tick pos=left,
title={},
x grid style={white!69.0196078431373!black},
xmajorgrids,
xmin=2, xmax=18,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={accuracy},
ymajorgrids,
ymin=0.358210862619808, ymax=0.872020766773163,
ytick style={color=black}
]
\addplot [semithick, blue, dashed, mark=*, mark size=3, mark options={solid}]
table {%
3 0.371505591054313
5 0.717651757188498
7 0.791134185303514
9 0.802715654952077
11 0.817791533546326
13 0.831869009584665
15 0.855431309904153
17 0.862020766773163
};
\addlegendentry{MSE}
\addplot [semithick, red, dashed, mark=*, mark size=3, mark options={solid}]
table {%
3 0.373602236421725
5 0.707468051118211
7 0.784544728434505
9 0.82577875399361
11 0.835563099041534
13 0.849640575079872
15 0.856729233226837
17 0.857827476038339
};
\addlegendentry{DeepLIFT Weighted MSE}
\addplot [semithick, green!50!black, dashed, mark=*, mark size=3, mark options={solid}]
table {%
3 0.368210862619808
5 0.703374600638978
7 0.77935303514377
9 0.831769169329074
11 0.847344249201278
13 0.852835463258786
15 0.855431309904153
17 0.862020766773163
};
\addlegendentry{Conductance Weighted MSE}

\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.97,0.03)}, anchor=south east, draw=white!80!black},
tick align=outside,
tick pos=left,
title={},
x grid style={white!69.0196078431373!black},
xmajorgrids,
xmin=2, xmax=18,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ymin=0.0190535143769968, ymax=0.594564696485623,
ytick style={color=black}
]
\addplot [semithick, blue, dashed, mark=*, mark size=3, mark options={solid}]
table {%
3 0.0290535143769968
5 0.196285942492013
7 0.345347444089457
9 0.376297923322684
11 0.431709265175719
13 0.485123801916933
15 0.492112619808307
17 0.577376198083067
};
\addlegendentry{MSE}
\addplot [semithick, red, dashed, mark=*, mark size=3, mark options={solid}]
table {%
3 0.0298522364217252
5 0.1997803514377
7 0.409145367412141
9 0.494808306709265
11 0.53594249201278
13 0.561801118210863
15 0.584464856230032
17 0.584564696485623
};
\addlegendentry{DeepLIFT Weighted MSE}
\addplot [semithick, green!50!black, dashed, mark=*, mark size=3, mark options={solid}]
table {%
3 0.0301517571884984
5 0.186801118210863
7 0.400459265175719
9 0.502196485623003
11 0.549720447284345
13 0.57198482428115
15 0.572683706070288
17 0.577975239616613
};
\addlegendentry{Conductance Weighted MSE}

\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.97,0.03)}, anchor=south east, draw=white!80!black},
tick align=outside,
tick pos=left,
title={},
x grid style={white!69.0196078431373!black},
xlabel={number of quantization levels},
xmajorgrids,
xmin=2, xmax=18,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={accuracy},
ymajorgrids,
ymin=0.429596645367412, ymax=0.894185303514377,
ytick style={color=black}
]
\addplot [semithick, blue, dashed, mark=*, mark size=3, mark options={solid}]
table {%
3 0.439596645367412
5 0.706170127795527
7 0.762979233226837
9 0.803115015974441
11 0.819388977635783
13 0.809804313099042
15 0.865015974440895
17 0.866014376996805
};
\addlegendentry{MSE}
\addplot [semithick, red, dashed, mark=*, mark size=3, mark options={solid}]
table {%
3 0.452376198083067
5 0.728334664536741
7 0.788738019169329
9 0.848642172523962
11 0.86172124600639
13 0.870706869009585
15 0.865814696485623
17 0.884185303514377
};
\addlegendentry{DeepLIFT Weighted MSE}
\addplot [semithick, green!50!black, dashed, mark=*, mark size=3, mark options={solid}]
table {%
3 0.444588658146965
5 0.719149361022364
7 0.793730031948882
9 0.843350638977636
11 0.851238019169329
13 0.877296325878594
15 0.873801916932907
17 0.879193290734824
};
\addlegendentry{Conductance Weighted MSE}

\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.97,0.03)}, anchor=south east, draw=white!80!black},
tick align=outside,
tick pos=left,
title={},
x grid style={white!69.0196078431373!black},
xlabel={number of quantization levels},
xmajorgrids,
xmin=2, xmax=18,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ymin=0.0195527156549521, ymax=0.616829073482428,
ytick style={color=black}
]
\addplot [semithick, blue, dashed, mark=*, mark size=3, mark options={solid}]
table {%
3 0.0358426517571885
5 0.275858626198083
7 0.394768370607029
9 0.431309904153355
11 0.461561501597444
13 0.48861821086262
15 0.541533546325879
17 0.594748402555911
};
\addlegendentry{MSE}
\addplot [semithick, red, dashed, mark=*, mark size=3, mark options={solid}]
table {%
3 0.0315495207667732
5 0.320287539936102
7 0.45547124600639
9 0.539337060702875
11 0.566393769968051
13 0.581569488817891
15 0.606829073482428
17 0.599241214057508
};
\addlegendentry{DeepLIFT Weighted MSE}
\addplot [semithick, green!50!black, dashed, mark=*, mark size=3, mark options={solid}]
table {%
3 0.0295527156549521
5 0.314197284345048
7 0.457767571884984
9 0.54073482428115
11 0.58236821086262
13 0.578474440894569
15 0.590255591054313
17 0.600938498402556
};
\addlegendentry{Conductance Weighted MSE}
\end{groupplot}

\end{tikzpicture}


==> figures/vgg16.tex <==
% This file was created by tikzplotlib v0.9.1.
\usepackage{tikz}
\usepackage{tikzscale}
\usetikzlibrary{shapes.geometric, arrows, shadows, positioning}
\begin{document}
\begin{tikzpicture}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={number of quantization levels},
xmajorgrids,
xmin=2, xmax=18,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={accuracy},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black}
]
\addplot [semithick, blue, dashed, mark=*, mark size=3, mark options={solid}]
table {%
4 0
6 0.1704
8 0.404
10 0.4916
12 0.5148
14 0.5024
16 0.5292
};
\addlegendentry{MSE}
\addplot [semithick, red, dashed, mark=*, mark size=3, mark options={solid}]
table {%
4 0
6 0.1128
8 0.5016
10 0.6044
12 0.6652
14 0.668
16 0.6652
};
\addlegendentry{DeepLIFT Weighted MSE}
\end{axis}

\end{tikzpicture}
\end{document}


==> head/bibgraph.tex <==
\addbibresource[label=primary]{references.bib}

\ifx\squeeze\empty
  \renewcommand*{\bibfont}{\scalefont{0.655}}
%\else
\fi

% % Bigger abbreviations (URL, ISBN, DOI)
% \renewcommand{\mkbibacro}[1]{%
%   \textls[55]{\scalefont{0.95}#1}\isdot}
%
% % Print pagetotal for "inproceedings"
% \DeclareFieldFormat[inproceedings]{pagetotal}{\mkpagetotal[pagination]{#1}}
% \renewbibmacro*{chapter+pages}{%
%   \printfield{chapter}%
%   \setunit{\bibpagespunct}%
%   \printfield{pages}%
%   \setunit{\bibpagespunct}%
%   \printfield{pagetotal}%
%   \newunit}
%
% % Display pagetotal for "article"
% \DeclareFieldFormat[article]{pagetotal}{\mkpagetotal[pagination]{#1}}
% \renewbibmacro*{note+pages}{%
%   \printfield{note}%
%   \setunit{\bibpagespunct}%
%   \printfield{pages}%
%   \setunit{\bibpagespunct}%
%   \printfield{pagetotal}%
%   \newunit}

% \DeclareFieldFormat{titlecase}{\MakeTitleCase{#1}}
% \newrobustcmd{\MakeTitleCase}[1]{%
%   \ifthenelse{\ifcurrentfield{booktitle}\OR\ifcurrentfield{booksubtitle}%
%     \OR\ifcurrentfield{maintitle}\OR\ifcurrentfield{mainsubtitle}%
%     \OR\ifcurrentfield{journaltitle}\OR\ifcurrentfield{journalsubtitle}%
%     \OR\ifcurrentfield{issuetitle}\OR\ifcurrentfield{issuesubtitle}%
%     \OR\ifentrytype{book}\OR\ifentrytype{mvbook}\OR\ifentrytype{bookinbook}%
%     \OR\ifentrytype{booklet}\OR\ifentrytype{suppbook}%
%     \OR\ifentrytype{collection}\OR\ifentrytype{mvcollection}%
%     \OR\ifentrytype{suppcollection}\OR\ifentrytype{manual}%
%     \OR\ifentrytype{periodical}\OR\ifentrytype{suppperiodical}%
%     \OR\ifentrytype{proceedings}\OR\ifentrytype{mvproceedings}%
%     \OR\ifentrytype{reference}\OR\ifentrytype{mvreference}%
%     \OR\ifentrytype{report}\OR\ifentrytype{thesis}}
%     {#1}
%     {\MakeSentenceCase{#1}}}


==> head/graphics.tex <==
\graphicspath{{figures/}}

\usetikzlibrary{external}
%\tikzset{external/mode=list and make}
\tikzexternalize[prefix=figures/]

\usepgfplotslibrary{units}
\pgfplotsset{compat=newest}


==> head/listings.tex <==
\usepackage{calc}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{scalefnt}

\makeatletter

\lstset{%
  captionpos=b,
  tabsize=2,
  numbers=left, xleftmargin=1.1em, framexleftmargin=1.2em,
  numbersep=3pt,
  basicstyle=\ttfamily\lst@ifdisplaystyle\scalefont{.75}\fi,
  numberstyle=\ttfamily\scalefont{.9},
  keywordstyle=\color{RoyalBlue},
  commentstyle=\color{green!50!black},
  stringstyle=\color{red},
  keepspaces=true,
  showstringspaces=false,
  breaklines=true,
  mathescape=true,
}


\lstnewenvironment{lstinlinelisting}[1][]{%
  \lstset{frame=none,numbers=none,aboveskip=\medskipamount,belowskip=\medskipamount,#1}%
}{}

\newcommand{\lstinputinlinelisting}[2][]{%
  \lstinputlisting[frame=none,numbers=none,aboveskip=\medskipamount,belowskip=\medskipamount,#1]{#2}%
}%

% patch lstinline to also work in mathmode with ttfamily
\expandafter\patchcmd\csname \string\lstinline\endcsname{%
    \leavevmode
    \bgroup
}{%
    \leavevmode
    \ifmmode\hbox\fi
    \bgroup
}{}{%
    \typeout{Patching of \string\lstinline\space failed!}%
}

\def\lst{\lstinline}
\def\print#1{\pgfmathparse{#1}\pgfmathresult}
\newcommand{\tikzmark}[1]{\tikz[overlay,remember picture] \node (#1) {};}
\newcommand*{\DrawArrow}[3][]{%
    % #1 = draw options
    % #2 = left point
    % #3 = right point
    \begin{tikzpicture}[overlay,remember picture]%
        \draw [-stealth,opacity=0.5,#1] ($(#2)-(0.2em,-0.4ex)$) to ($(#3)-(0.2em,-0.4ex)$);%
    \end{tikzpicture}%
}%

% ----- BOOK-STYLE LISTINGS - COMMENT FOR NORMAL LISTINGS -----
%% For fancy listing captions, we need to load the caption package, which will
%% override the template style for tables and figures. The following four steps
%% will circumvent this issue.
%
%% 1. Store original caption command before it gets overridden by caption package
%\let\originalmakecaption\@makecaption
%
%% 2. Load caption package
%\usepackage{caption}
%
%% 3. Store caption packages caption command before defining our own
%\let\captionsmakecaption\@makecaption
%
%% 4. Define our own caption command
%\long\def\@makecaption#1#2{%
%  \ifthenelse{\equal{\@captype}{lstlisting}}{%
%    % This is a listing, use caption packages caption command
%    \captionsmakecaption{#1}{#2}%
%  }{%
%    % This is not a listing, use the templates original caption command
%    \originalmakecaption{#1}{#2}%
%  }
%}
%
%\definecolor{captiongray}{rgb}{0.56470, 0.56470, 0.56470}
%
%\newlength{\captionskip}
%\newlength{\captionlength}
%\DeclareCaptionFont{white}{\color{white}}
%\DeclareCaptionFormat{listing}{%
%  \settodepth{\captionskip}{g}%
%  \settowidth{\captionlength}{#1#2}%
%  \colorbox{captiongray}{%
%    \hspace{.5\captionskip}%
%    \parbox{\linewidth-.85em-\captionskip}{%
%      \parbox[t]{\captionlength}{\strut#1#2}%
%      \parbox[t]{\linewidth-.85em-\captionskip-\captionlength}{#3}%
%      \vspace{-\captionskip}} % vertically align
%    \hspace{.5\captionskip}}}
%
%\captionsetup[lstlisting]{%
%  format=listing,%
%  singlelinecheck=false,%
%  margin=0pt,%
%  font={white,sf,bf,footnotesize},%
%  labelsep=colon}
%
%\lstset{%
%  frame=b,
%  captionpos=t,
%  basicstyle=\ttfamily\lst@ifdisplaystyle\scalefont{.75}\fi,
%  numberstyle=\ttfamily\scalefont{.9},
%  keywordstyle=\color{RoyalBlue},
%  commentstyle=\color{green!50!black},
%  stringstyle=\color{red},
%  rulecolor=\color{captiongray},
%  aboveskip=0pt,
%  belowskip=0pt,
%  backgroundcolor=\color{white},
%  belowcaptionskip=3pt,
%  xleftmargin=17pt,
%  framexleftmargin=17pt,
%  framexrightmargin=0pt,
%  framexbottommargin=0pt,
%}
% ----- END OF BOOK-STYLE LISTINGS - COMMENT FOR NORMAL LISTINGS -----

\makeatother

\lstdefinelanguage{OpenVX}{%
  language=C++,
  morekeywords={vxCreateImage, vxCreateVirtualImage, vxReleaseContext,
                vxCreateGraph, vxVerifyGraph, vxProcessGraph, vxCreateContext,
                vxGaussian3x3Node, vxSobel, vxSobel3x3Node, vxMagnitudeNode, vxPhaseNode,
                vxChannelExtractNode, vxAddParameterToKernel,vxCreateScalar,
                vxSetParameterByIndex, vxFinalizeKernel, vxCreateGenericNode,
                vxThresholdNode, vxCreateMatrix, vxCopyMatrix
                },
  keywords=[2]{vx_image, vx_context, vx_graph, VX_SUCCESS, VX_DF_IMAGE_VIRT, VX_DF_IMAGE_UYVY,
              VX_DF_IMAGE_S16, VX_DF_IMAGE_U8, VX_CHANNEL_Y, vx_matrix, vx_node
              },
  keywords=[3]{vxHipaccKernel, DOMVX_LOCAL},
  %keywordstyle=[2]{\color{Cerulean}\bfseries}
  keywordstyle=[2]{\color{Magenta}\bfseries},
  keywordstyle=[3]{\color{blue}\bfseries}
}


\lstdefinelanguage{HIPAcc}{%
  language=C++,
  morekeywords={size_t, uchar, ushort, uint, uchar4, char4, ushort4, short4,
    uint4, int4, float4, double4},
  keywords=[2]{Image, Accessor, Kernel, IterationSpace, Mask, BoundaryCondition,
    Boundary, CLAMP, MIRROR, UNDEFINED, REPEAT, CONSTANT, output, convolve,
    iterate, reduce, Reduce, SUM, MIN, MAX, PROD, MEDIAN Domain},
  %keywordstyle=[2]{\color{Cerulean}\bfseries}
  keywordstyle=[2]{\color{blue}\bfseries}
}

\lstdefinestyle{CUDA}{%
  language=C++,
  morekeywords={size_t, uchar, ushort, uint, uchar4, char4, ushort4, short4,
    uint4, int4, float4, double4},
  otherkeywords=[2]{>>>,<<<,[,]},
  alsoletter=[2]{.},
  keywords=[2]{__device__, __host__, __global__, __constant__, __shared__, dim3,
    blockIdx.x, blockIdx.y, blockDim.x, blockDim.y, blockDim.z, threadIdx.x,
    threadIdx.y, threadIdx.z, gridDim.x, gridDim.y, warpSize, __syncthreads,
    __sinf, __cosf, __expf, cudaMalloc, cudaMemset, cudaFree, cudaMemcpy,
    cudaMemcpyHostToDevice, cudaMemcpyDeviceToHost, cudaMemcpyDeviceToDevice,
    tex1Dfetch, tex2D, surf2Dwrite},
  keywordstyle=[2]{\color{blue}\bfseries}
}

\lstdefinestyle{OpenCL}{%
  language=C,
  morekeywords={size_t, uchar, ushort, uint, uchar4, char4, ushort4, short4,
    uint4, int4, float4, double4},
  keywords=[2]{__kernel, __global, __constant, __local, get_num_groups,
    get_local_size, get_group_id, get_local_id, get_global_id, get_global_size,
    barrier, mem_fence, CLK_GLOBAL_MEM_FENCE, CLK_LOCAL_MEM_FENCE,
    read_mem_fence, write_mem_fence, read_imagef, write_imagef},
  keywordstyle=[2]{\color{Cerulean}\bfseries}
}



==> head/todonotes.tex <==
% Set margin dimensions
\ifx\final\empty\else\ifx\print\empty\else%
  \marginparsep 0.5em
  \marginparwidth 3.5pc
\fi\fi

\makeatletter

% Patch todo to handle TikZ externalize
\renewcommand{\todo}[2][color=Cerulean!20]{%
  \ifx\final\empty\else\ifx\print\empty\else%
    \ifx\tikzexternaldisable\undefined\else%
      \tikzexternaldisable%
    \fi
    \@todo[size=\scriptsize,caption={#2},#1]{#2}%
    \ifx\tikzexternalenable\undefined\else%
      \tikzexternalenable%
    \fi
  \fi\fi}

% Patch missingfigure to handle TikZ externalize
\let\MissingFigure\missingfigure
\newcommand{\MyMissingFigure}[2][]{%
  \tikzexternaldisable%
  \MissingFigure[#1]{#2}%
  \tikzexternalenable}%
\let\missingfigure\MyMissingFigure

\makeatother


==> head/typeset.tex <==
%uncomment in main: \def\squeeze{}
\newlength\nspace
\newlength\fspace
\newlength\subfspace
\newlength\lstspaceAbove
\newlength\lstspaceBelow
\newlength\lstinlinespace
\newlength\spaceoffset
\newlength\spaceoffsetneg

\newcommand{\eqsize}{\small}

% common
\setlength\lstinlinespace{0.25\baselineskip} % Listing: inlined

\ifx\squeeze\empty
    % Line spacing
    \linespread{0.9601}

    % Margins
    %\usepackage[left=1.5cm, right=1.5cm, top=1.5cm, bottom=2.35cm]{geometry}
    %\usepackage[left=1.7cm, right=1.7cm, top=1.7cm, bottom=2.65cm]{geometry}

    % Font expansion
    \SetExpansion[shrink=50]{encoding={OT1,T1,TS1}}{}

    %figure spacing
    \setlength\medskipamount{\smallskipamount} % shouldn't be used in this paper
    \setlength\nspace{-1ex} % text after caption
    \setlength\fspace{-3.2ex}  % caption after figure
    \setlength\subfspace{-0.6ex}  % caption after figure
    \setlength\spaceoffset{0.6ex}  % caption after figure
    \setlength\spaceoffsetneg{-0.6ex}  % caption after figure

    % Algorithm spacing
    \newcommand{\negskip}{\vspace{-1ex}}
    \SetAlgoSkip{negskip}

    % Listing spacing (With captions)
    %\setlength\lstspaceAbove{\smallskipamount}
    %\setlength\lstspaceBelow{\smallskipamount}
    \setlength\lstspaceAbove{0ex}
    \setlength\lstspaceBelow{-2.5ex}

    % Global font squeeze
    \def\fontsqueezefactor{0.967}
    %\def\fontsqueezefactor{1}

    % Caption size
    %\newcommand{\captionfontsize}{\small}
    \newcommand{\captionfontsize}{}
\else
    % Line spacing
    \linespread{1.00}

    %figure spacing (Do not touch)
    \setlength\nspace{0ex} % text after caption
    \setlength\fspace{0ex}  % caption after figure
    \setlength\subfspace{0ex}  % caption after figure
    \setlength\spaceoffset{0ex}  % caption after figure

    % Listing spacing (With captions)
    \setlength\lstspaceAbove{\medskipamount}
    \setlength\lstspaceBelow{\medskipamount}

    % Font expansion
    \SetExpansion[stretch=20, shrink=20]{encoding={OT1,T1,TS1}}{}

    % Caption size
    \newcommand{\captionfontsize}{}%\small}
\fi

% Abbreviations
\newcommand{\ie}{\mbox{i.e.,}\xspace}
\newcommand{\eg}{\mbox{e.g.,}\xspace}

% Enable copy&paste and search for words including ligatures
\input glyphtounicode.tex
\pdfgentounicode=1

% space after inlined listings
\newcommand{\lstinlineskip}{\vskip \lstinlinespace}

% Add thin space to xspace exception list
\xspaceaddexceptions{\,}

% Use normal font style for URLs
\urlstyle{same}

% Use abbreviation for references to equations
\crefname{equation}{eq.}{eqs.}
\Crefname{equation}{Eq.}{Eqs.}

% Always use capitalized version of cref
\let\cref\Cref

% Shortcut to highlight code within text
\newcommand{\code}[1]{\texttt{#1}}

